Optimizing intermodal transportation networks at scale via column generation

In light of the need for design and analysis of intermodal transportation systems, we propose an algorithmic framework to determine the system optimum of an intermodal transportation system. To this end, we model an intermodal transportation system by combining two core principles of network optimization - layered-graph structures and (partially) time-expanded networks - to formulate our problem on a graph that allows us to implicitly encode problem specific constraints related to intermodality. This enables us to solve a standard integer minimum-cost multi-commodity flow problem to obtain the system optimum for an intermodal transportation system. To solve this integer minimum-cost multi-commodity flow problem efficiently, we present a column generation approach to find continuous minimum-cost multi-commodity flow solutions, which we combine with a price-and-branch procedure to obtain integer solutions. To speed up our column generation, we further develop a pricing filter and an admissible distance approximation to utilize the $A^*$ algorithm for solving the pricing problems. We show the efficiency of our framework by applying it to a real-world case study for the city of Munich, where we solve instances with up to 56,295 passengers to optimality, and show that the computation time of our algorithm can be reduced by up to 60\% through the use of our pricing filter and by up to additional 90\% through the use of the $A^*$-based pricing algorithm.

==> Figures/runtime_bus.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{dimgray111}{RGB}{111,111,111}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{skyblue147200222}{RGB}{147,200,222}
\definecolor{whitesmoke239240241}{RGB}{239,240,241}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Subset},
xmin=-0.5, xmax=8.5,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9},
y grid style={darkgray176},
ylabel={Runtime in seconds},
ymin=-41.1191596150398, ymax=1381.1910897851,
ytick style={color=black}
]
\path [draw=dimgray111, fill=whitesmoke239240241, semithick]
(axis cs:-0.396,26.0278756022453)
--(axis cs:-0.004,26.0278756022453)
--(axis cs:-0.004,40.2216595411301)
--(axis cs:-0.396,40.2216595411301)
--(axis cs:-0.396,26.0278756022453)
--cycle;
\path [draw=dimgray111, fill=skyblue147200222, semithick]
(axis cs:0.004,44.082723736763)
--(axis cs:0.396,44.082723736763)
--(axis cs:0.396,54.5207988023758)
--(axis cs:0.004,54.5207988023758)
--(axis cs:0.004,44.082723736763)
--cycle;
\path [draw=dimgray111, fill=whitesmoke239240241, semithick]
(axis cs:0.604,53.0346139073372)
--(axis cs:0.996,53.0346139073372)
--(axis cs:0.996,76.9802179932594)
--(axis cs:0.604,76.9802179932594)
--(axis cs:0.604,53.0346139073372)
--cycle;
\path [draw=dimgray111, fill=skyblue147200222, semithick]
(axis cs:1.004,110.656690955162)
--(axis cs:1.396,110.656690955162)
--(axis cs:1.396,121.476613044739)
--(axis cs:1.004,121.476613044739)
--(axis cs:1.004,110.656690955162)
--cycle;
\path [draw=dimgray111, fill=whitesmoke239240241, semithick]
(axis cs:1.604,106.084294557571)
--(axis cs:1.996,106.084294557571)
--(axis cs:1.996,124.170395612717)
--(axis cs:1.604,124.170395612717)
--(axis cs:1.604,106.084294557571)
--cycle;
\path [draw=dimgray111, fill=skyblue147200222, semithick]
(axis cs:2.004,180.426746606827)
--(axis cs:2.396,180.426746606827)
--(axis cs:2.396,213.843363761902)
--(axis cs:2.004,213.843363761902)
--(axis cs:2.004,180.426746606827)
--cycle;
\path [draw=dimgray111, fill=whitesmoke239240241, semithick]
(axis cs:2.604,144.031060159206)
--(axis cs:2.996,144.031060159206)
--(axis cs:2.996,196.20437258482)
--(axis cs:2.604,196.20437258482)
--(axis cs:2.604,144.031060159206)
--cycle;
\path [draw=dimgray111, fill=skyblue147200222, semithick]
(axis cs:3.004,269.98458302021)
--(axis cs:3.396,269.98458302021)
--(axis cs:3.396,324.797195911407)
--(axis cs:3.004,324.797195911407)
--(axis cs:3.004,269.98458302021)
--cycle;
\path [draw=dimgray111, fill=whitesmoke239240241, semithick]
(axis cs:3.604,217.589021742344)
--(axis cs:3.996,217.589021742344)
--(axis cs:3.996,257.497653186321)
--(axis cs:3.604,257.497653186321)
--(axis cs:3.604,217.589021742344)
--cycle;
\path [draw=dimgray111, fill=skyblue147200222, semithick]
(axis cs:4.004,365.301903903484)
--(axis cs:4.396,365.301903903484)
--(axis cs:4.396,446.865532696247)
--(axis cs:4.004,446.865532696247)
--(axis cs:4.004,365.301903903484)
--cycle;
\path [draw=dimgray111, fill=whitesmoke239240241, semithick]
(axis cs:4.604,309.760082960129)
--(axis cs:4.996,309.760082960129)
--(axis cs:4.996,386.271408140659)
--(axis cs:4.604,386.271408140659)
--(axis cs:4.604,309.760082960129)
--cycle;
\path [draw=dimgray111, fill=skyblue147200222, semithick]
(axis cs:5.004,612.74171090126)
--(axis cs:5.396,612.74171090126)
--(axis cs:5.396,708.914951205254)
--(axis cs:5.004,708.914951205254)
--(axis cs:5.004,612.74171090126)
--cycle;
\path [draw=dimgray111, fill=whitesmoke239240241, semithick]
(axis cs:5.604,372.022395372391)
--(axis cs:5.996,372.022395372391)
--(axis cs:5.996,407.531775951385)
--(axis cs:5.604,407.531775951385)
--(axis cs:5.604,372.022395372391)
--cycle;
\path [draw=dimgray111, fill=skyblue147200222, semithick]
(axis cs:6.004,714.970948934555)
--(axis cs:6.396,714.970948934555)
--(axis cs:6.396,804.97754240036)
--(axis cs:6.004,804.97754240036)
--(axis cs:6.004,714.970948934555)
--cycle;
\path [draw=dimgray111, fill=whitesmoke239240241, semithick]
(axis cs:6.604,510.46615421772)
--(axis cs:6.996,510.46615421772)
--(axis cs:6.996,531.248596429825)
--(axis cs:6.604,531.248596429825)
--(axis cs:6.604,510.46615421772)
--cycle;
\path [draw=dimgray111, fill=skyblue147200222, semithick]
(axis cs:7.004,900.730874478817)
--(axis cs:7.396,900.730874478817)
--(axis cs:7.396,921.771727740765)
--(axis cs:7.004,921.771727740765)
--(axis cs:7.004,900.730874478817)
--cycle;
\path [draw=dimgray111, fill=whitesmoke239240241, semithick]
(axis cs:7.604,600.310883581638)
--(axis cs:7.996,600.310883581638)
--(axis cs:7.996,670.725666224957)
--(axis cs:7.604,670.725666224957)
--(axis cs:7.604,600.310883581638)
--cycle;
\path [draw=dimgray111, fill=skyblue147200222, semithick]
(axis cs:8.004,1111.01089715958)
--(axis cs:8.396,1111.01089715958)
--(axis cs:8.396,1131.66493725777)
--(axis cs:8.004,1131.66493725777)
--(axis cs:8.004,1111.01089715958)
--cycle;
\draw[draw=dimgray111,fill=whitesmoke239240241,line width=0.3pt] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar,ybar legend,draw=dimgray111,fill=whitesmoke239240241,line width=0.3pt}
\addlegendentry{On}

\draw[draw=dimgray111,fill=skyblue147200222,line width=0.3pt] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar,ybar legend,draw=dimgray111,fill=skyblue147200222,line width=0.3pt}
\addlegendentry{Off}

\addplot [semithick, dimgray111, forget plot]
table {%
-0.2 26.0278756022453
-0.2 23.5313062667847
};
\addplot [semithick, dimgray111, forget plot]
table {%
-0.2 40.2216595411301
-0.2 47.1337604522705
};
\addplot [semithick, dimgray111, forget plot]
table {%
-0.298 23.5313062667847
-0.102 23.5313062667847
};
\addplot [semithick, dimgray111, forget plot]
table {%
-0.298 47.1337604522705
-0.102 47.1337604522705
};
\addplot [semithick, dimgray111, forget plot]
table {%
0.2 44.082723736763
0.2 38.7160239219666
};
\addplot [semithick, dimgray111, forget plot]
table {%
0.2 54.5207988023758
0.2 65.0901112556458
};
\addplot [semithick, dimgray111, forget plot]
table {%
0.102 38.7160239219666
0.298 38.7160239219666
};
\addplot [semithick, dimgray111, forget plot]
table {%
0.102 65.0901112556458
0.298 65.0901112556458
};
\addplot [semithick, dimgray111, forget plot]
table {%
0.8 53.0346139073372
0.8 48.7842261791229
};
\addplot [semithick, dimgray111, forget plot]
table {%
0.8 76.9802179932594
0.8 90.697313785553
};
\addplot [semithick, dimgray111, forget plot]
table {%
0.702 48.7842261791229
0.898 48.7842261791229
};
\addplot [semithick, dimgray111, forget plot]
table {%
0.702 90.697313785553
0.898 90.697313785553
};
\addplot [semithick, dimgray111, forget plot]
table {%
1.2 110.656690955162
1.2 104.806071519852
};
\addplot [semithick, dimgray111, forget plot]
table {%
1.2 121.476613044739
1.2 134.191674947739
};
\addplot [semithick, dimgray111, forget plot]
table {%
1.102 104.806071519852
1.298 104.806071519852
};
\addplot [semithick, dimgray111, forget plot]
table {%
1.102 134.191674947739
1.298 134.191674947739
};
\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=dimgray111}, only marks, forget plot]
table {%
1.2 76.8118605613708
};
\addplot [semithick, dimgray111, forget plot]
table {%
1.8 106.084294557571
1.8 82.8600149154663
};
\addplot [semithick, dimgray111, forget plot]
table {%
1.8 124.170395612717
1.8 150.364614009857
};
\addplot [semithick, dimgray111, forget plot]
table {%
1.702 82.8600149154663
1.898 82.8600149154663
};
\addplot [semithick, dimgray111, forget plot]
table {%
1.702 150.364614009857
1.898 150.364614009857
};
\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=dimgray111}, only marks, forget plot]
table {%
1.8 197.661225318909
};
\addplot [semithick, dimgray111, forget plot]
table {%
2.2 180.426746606827
2.2 143.877823829651
};
\addplot [semithick, dimgray111, forget plot]
table {%
2.2 213.843363761902
2.2 249.996301174164
};
\addplot [semithick, dimgray111, forget plot]
table {%
2.102 143.877823829651
2.298 143.877823829651
};
\addplot [semithick, dimgray111, forget plot]
table {%
2.102 249.996301174164
2.298 249.996301174164
};
\addplot [semithick, dimgray111, forget plot]
table {%
2.8 144.031060159206
2.8 139.038941383362
};
\addplot [semithick, dimgray111, forget plot]
table {%
2.8 196.20437258482
2.8 206.328284263611
};
\addplot [semithick, dimgray111, forget plot]
table {%
2.702 139.038941383362
2.898 139.038941383362
};
\addplot [semithick, dimgray111, forget plot]
table {%
2.702 206.328284263611
2.898 206.328284263611
};
\addplot [semithick, dimgray111, forget plot]
table {%
3.2 269.98458302021
3.2 224.508894681931
};
\addplot [semithick, dimgray111, forget plot]
table {%
3.2 324.797195911407
3.2 347.637128829956
};
\addplot [semithick, dimgray111, forget plot]
table {%
3.102 224.508894681931
3.298 224.508894681931
};
\addplot [semithick, dimgray111, forget plot]
table {%
3.102 347.637128829956
3.298 347.637128829956
};
\addplot [semithick, dimgray111, forget plot]
table {%
3.8 217.589021742344
3.8 206.835752487183
};
\addplot [semithick, dimgray111, forget plot]
table {%
3.8 257.497653186321
3.8 270.982366323471
};
\addplot [semithick, dimgray111, forget plot]
table {%
3.702 206.835752487183
3.898 206.835752487183
};
\addplot [semithick, dimgray111, forget plot]
table {%
3.702 270.982366323471
3.898 270.982366323471
};
\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=dimgray111}, only marks, forget plot]
table {%
3.8 321.008467197418
};
\addplot [semithick, dimgray111, forget plot]
table {%
4.2 365.301903903484
4.2 336.777513980865
};
\addplot [semithick, dimgray111, forget plot]
table {%
4.2 446.865532696247
4.2 507.392606735229
};
\addplot [semithick, dimgray111, forget plot]
table {%
4.102 336.777513980865
4.298 336.777513980865
};
\addplot [semithick, dimgray111, forget plot]
table {%
4.102 507.392606735229
4.298 507.392606735229
};
\addplot [semithick, dimgray111, forget plot]
table {%
4.8 309.760082960129
4.8 288.419535160065
};
\addplot [semithick, dimgray111, forget plot]
table {%
4.8 386.271408140659
4.8 392.265806674957
};
\addplot [semithick, dimgray111, forget plot]
table {%
4.702 288.419535160065
4.898 288.419535160065
};
\addplot [semithick, dimgray111, forget plot]
table {%
4.702 392.265806674957
4.898 392.265806674957
};
\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=dimgray111}, only marks, forget plot]
table {%
4.8 520.701917409897
};
\addplot [semithick, dimgray111, forget plot]
table {%
5.2 612.74171090126
5.2 537.552830219269
};
\addplot [semithick, dimgray111, forget plot]
table {%
5.2 708.914951205254
5.2 745.604617118835
};
\addplot [semithick, dimgray111, forget plot]
table {%
5.102 537.552830219269
5.298 537.552830219269
};
\addplot [semithick, dimgray111, forget plot]
table {%
5.102 745.604617118835
5.298 745.604617118835
};
\addplot [semithick, dimgray111, forget plot]
table {%
5.8 372.022395372391
5.8 370.544471263885
};
\addplot [semithick, dimgray111, forget plot]
table {%
5.8 407.531775951385
5.8 426.066930770874
};
\addplot [semithick, dimgray111, forget plot]
table {%
5.702 370.544471263885
5.898 370.544471263885
};
\addplot [semithick, dimgray111, forget plot]
table {%
5.702 426.066930770874
5.898 426.066930770874
};
\addplot [semithick, dimgray111, forget plot]
table {%
6.2 714.970948934555
6.2 701.358267784119
};
\addplot [semithick, dimgray111, forget plot]
table {%
6.2 804.97754240036
6.2 821.584753751755
};
\addplot [semithick, dimgray111, forget plot]
table {%
6.102 701.358267784119
6.298 701.358267784119
};
\addplot [semithick, dimgray111, forget plot]
table {%
6.102 821.584753751755
6.298 821.584753751755
};
\addplot [semithick, dimgray111, forget plot]
table {%
6.8 510.46615421772
6.8 492.398324489594
};
\addplot [semithick, dimgray111, forget plot]
table {%
6.8 531.248596429825
6.8 531.911300182343
};
\addplot [semithick, dimgray111, forget plot]
table {%
6.702 492.398324489594
6.898 492.398324489594
};
\addplot [semithick, dimgray111, forget plot]
table {%
6.702 531.911300182343
6.898 531.911300182343
};
\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=dimgray111}, only marks, forget plot]
table {%
6.8 441.870304822922
6.8 602.182353496552
6.8 566.404212474823
};
\addplot [semithick, dimgray111, forget plot]
table {%
7.2 900.730874478817
7.2 890.020228147507
};
\addplot [semithick, dimgray111, forget plot]
table {%
7.2 921.771727740765
7.2 922.866987943649
};
\addplot [semithick, dimgray111, forget plot]
table {%
7.102 890.020228147507
7.298 890.020228147507
};
\addplot [semithick, dimgray111, forget plot]
table {%
7.102 922.866987943649
7.298 922.866987943649
};
\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=dimgray111}, only marks, forget plot]
table {%
7.2 1182.16604018211
7.2 1048.33904004097
};
\addplot [semithick, dimgray111, forget plot]
table {%
7.8 600.310883581638
7.8 551.414462327957
};
\addplot [semithick, dimgray111, forget plot]
table {%
7.8 670.725666224957
7.8 711.767167329788
};
\addplot [semithick, dimgray111, forget plot]
table {%
7.702 551.414462327957
7.898 551.414462327957
};
\addplot [semithick, dimgray111, forget plot]
table {%
7.702 711.767167329788
7.898 711.767167329788
};
\addplot [semithick, dimgray111, forget plot]
table {%
8.2 1111.01089715958
8.2 1107.62679338455
};
\addplot [semithick, dimgray111, forget plot]
table {%
8.2 1131.66493725777
8.2 1133.31560587883
};
\addplot [semithick, dimgray111, forget plot]
table {%
8.102 1107.62679338455
8.298 1107.62679338455
};
\addplot [semithick, dimgray111, forget plot]
table {%
8.102 1133.31560587883
8.298 1133.31560587883
};
\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=dimgray111}, only marks, forget plot]
table {%
8.2 964.817253828049
8.2 1316.54062390327
};
\addplot [semithick, dimgray111, forget plot]
table {%
-0.396 31.6739937067032
-0.004 31.6739937067032
};
\addplot [semithick, dimgray111, forget plot]
table {%
0.004 48.2410128116608
0.396 48.2410128116608
};
\addplot [semithick, dimgray111, forget plot]
table {%
0.604 69.6084365844727
0.996 69.6084365844727
};
\addplot [semithick, dimgray111, forget plot]
table {%
1.004 114.639037847519
1.396 114.639037847519
};
\addplot [semithick, dimgray111, forget plot]
table {%
1.604 119.576555967331
1.996 119.576555967331
};
\addplot [semithick, dimgray111, forget plot]
table {%
2.004 197.543394565582
2.396 197.543394565582
};
\addplot [semithick, dimgray111, forget plot]
table {%
2.604 168.08328807354
2.996 168.08328807354
};
\addplot [semithick, dimgray111, forget plot]
table {%
3.004 293.407308697701
3.396 293.407308697701
};
\addplot [semithick, dimgray111, forget plot]
table {%
3.604 242.60850250721
3.996 242.60850250721
};
\addplot [semithick, dimgray111, forget plot]
table {%
4.004 428.36933016777
4.396 428.36933016777
};
\addplot [semithick, dimgray111, forget plot]
table {%
4.604 360.247135639191
4.996 360.247135639191
};
\addplot [semithick, dimgray111, forget plot]
table {%
5.004 627.58005464077
5.396 627.58005464077
};
\addplot [semithick, dimgray111, forget plot]
table {%
5.604 381.309901952744
5.996 381.309901952744
};
\addplot [semithick, dimgray111, forget plot]
table {%
6.004 737.547736644745
6.396 737.547736644745
};
\addplot [semithick, dimgray111, forget plot]
table {%
6.604 525.001151442528
6.996 525.001151442528
};
\addplot [semithick, dimgray111, forget plot]
table {%
7.004 909.551081418991
7.396 909.551081418991
};
\addplot [semithick, dimgray111, forget plot]
table {%
7.604 648.536518096924
7.996 648.536518096924
};
\addplot [semithick, dimgray111, forget plot]
table {%
8.004 1125.88824319839
8.396 1125.88824319839
};
\end{axis}

\end{tikzpicture}


==> resources/commands.tex <==
%% additional user defined commands

